BLIP-2: Bootstrapping Language-Image Pre-training with Frozen Image Encoders and Large Language Models

The cost of vision-and-language pre-training has become increasingly prohibitive due to end-to-end training of large-scale models. This paper proposes BLIP-2, a generic and efficient pre-training strategy that bootstraps vision-language pre-training from off-the-shelf frozen pre-trained image encoders and frozen large language models. BLIP-2 bridges the modality gap with a lightweight Querying Transformer, which is pre-trained in two stages. The first stage bootstraps vision-language representation learning from a frozen image encoder. The second stage bootstraps vision-to-language generative learning from a frozen language model. BLIP-2 achieves state-of-the-art performance on various vision-language tasks, despite having significantly fewer trainable parameters than existing methods. For example, our model outperforms Flamingo80B by 8.7% on zero-shot VQAv2 with 54x fewer trainable parameters. We also demonstrate the model's emerging capabilities of zero-shot image-to-text generation that can follow natural language instructions.

==> table/param_count.tex <==
\begin{table*}[!t]
    % \aboverulesep = 0.48mm
    % \belowrulesep = 0.48mm
    % \small
	\centering	
    \setlength\tabcolsep{5pt}
	\resizebox{1\textwidth}{!}{%
	\begin{tabular}	{l | l l l l l l l}
	Models & ALBEF~\cite{ALBEF} & BLIP~\cite{blip} & OFA~\cite{ofa}& SimVLM~\cite{simvlm}& BEIT-3~\cite{beit3} & Flamingo~\cite{flamingo}  & BLIP-2\\
	\toprule
	\#Trainable params & 233M & 583M & 930M & 1.4B  & 1.9B& 10.2B & \textbf{199M}\\
	\#Images & 14M & 129M & 54M &1.8B & 29M& 2.4B & \textbf{14M}\\
	\#Pre-train iters & & & & &1M & 1.7M & 150k \\
	\bottomrule

	\end{tabular}
}
 \vspace{-1ex}
	\caption
	{
	\small	
		Number of
	}
	\vspace{-1ex}
	\label{tbl:param_count}
\end{table*}	

==> table/retrieval_caption.tex <==
\begin{table*}[!t]
    % \aboverulesep = 0.48mm
    % \belowrulesep = 0.48mm
    \small
	\centering	
 \setlength\tabcolsep{3pt}
%  \vspace{-3ex}
	\resizebox{\textwidth}{!}{%
	\begin{tabular}	{l l l |  c  c  c  c | c  c  c  c | c  c }
		\toprule	 	
	 \multirow{3}{*}{Model} & \multirow{3}{*}{\makecell[l]{\#Trainable \\ Params}}& \multirow{3}{*}{\makecell[l]{Pre-train \\ \#Images}} &\multicolumn{4}{c|}{Flickr30K Retrieval (ZS) }   & \multicolumn{4}{c|}{COCO Retrieval (FT)} & \multicolumn{2}{c}{COCO Caption (FT)}\\
	 & &  &  \multicolumn{2}{c}{TR}& \multicolumn{2}{c|}{IR} &  \multicolumn{2}{c}{TR}& \multicolumn{2}{c|}{IR}&\multicolumn{2}{c}{Karpathy test}\\
	     
	& & & R@1 &R@5& R@1 &R@5& R@1 &R@5& R@1 &R@5& B@4 & C\\
	\midrule  
    \multicolumn{6}{l}{\textit{~~Encoder-only models}} \\
	UNITER\dag~\cite{uniter} & 303M & 4M 
	& 83.6 & 95.7 & 68.7 & 89.2 
	&65.7  &88.6 &52.9 &79.9 & \multicolumn{2}{c}{\multirow{4}{*}{\xmark}}
	\\    
	ALIGN~\cite{align} & 820M & 1.8B 
	& 88.6 &  98.7 & 75.7 & 93.8 
	& 77.0 & 93.5 &  59.9 & 83.3 
	\\    
	FILIP~\cite{filip} &417M & 339M
	&89.8& 99.2 &75.0 &93.4
	& 78.9& 94.4& 61.2& 84.3
	\\
	Florence~\cite{florence}& 893M &900M 
	&90.9& 99.1 &76.7& 93.6
	& 81.8 & 95.2  & 63.2 & 85.7 
	\\
	ALBEF~\cite{ALBEF} &233M & 14M 
	& 94.1 & 99.5  & 82.8 & 96.3 
	&77.6 & 94.3 & 60.7& 84.3 
	\\

	\midrule  
    \multicolumn{6}{l}{\textit{~~Vision-to-Language generative models}} \\
	    SimVLM~\cite{simvlm} & $\sim$1.4B$^\ast$ & 1.8B &\multicolumn{4}{c|}{\multirow{4}{*}{\xmark}}& \multicolumn{4}{c|}{\multirow{4}{*}{\xmark}}
	    & 40.6 &  143.3\\    
	   Flamingo~\cite{flamingo} & 10.6B$^\ast$ & 2.4B&  
	   &   &  & &   & &  &  
	   & - & 138.1\\
	   LEMON\dag~\cite{lemon} & 675M &200M &  
	   &   &  & &   & &  &  
	   &  42.6 & 145.5 \\		   
	   OFA~\cite{ofa} & 930M & 54M$^\ast$ &  
	   &   &  & &   & &  &  
	   &  43.9 & 145.3\\    
	 \midrule
    \multicolumn{6}{l}{\textit{~~Unified models}} \\	   
	OSCAR\dag~\cite{oscar} & 345M & 4M 
	& - & -  & - & - 
	& 70.0 & 91.1  &  54.0 & 80.8 
	& 37.4&127.8\\
   VinVL\dag~\cite{vinvl} & 345M &5.7M 
   & - & -  & - & - 
	&  75.4 & 92.9 & 58.8 & 83.5 
	& 37.4&127.8\\	
    BLIP~\cite{blip} &446M  & 129M 
    & 96.7 & 100.0& 86.7 & 97.3 
    & 82.4 & 95.4& 65.1 & 86.3 & 40.4 & 136.7
    \\    
	BEIT-3\cite{beit3} &1.9B$^\ast$ & 29M
	&94.9 & 99.9 & 81.5 & 95.6 
	& 84.8 & 96.5 & 67.2& 87.7 & 44.1 & 147.6
	\\    
	\midrule
	\multicolumn{6}{l}{\textit{~~Multi-task unified model}} \\	   
    BLIPv2-GMT & 490M & 14M 
     & \textbf{97.4} & \textbf{100.0}  &  \textbf{87.7}& \textbf{97.6} 
    & 83.0 & 95.9 & 66.3 & 86.3& 40.3 & 137.8\\  
    \bottomrule
	\end{tabular}
	}
	\vspace{-1ex}
	\caption
	{
	\small
	Comparison with state-of-the-art models on image-text retrieval and image captioning tasks. ZS: zero-shot. FT: fine-tuned. TR / IR@1: recall@1 for text retrieval / image retrieval. B@4: BLEU-4@4. C:CIDEr.\\
	Unified models: pre-trained models that can be fine-tuned on either understanding or generation task.
	\\
	Multi-task unified model: BLIPv2-GMT can be fine-tuned on both understanding and generation tasks at the same time.
	\\
	Methods with \dag~have slow inference speed due to the use of object detector on high resolution images.
	OFA~\cite{ofa} requires a large amount of high-quality human-annotated data during pre-training.
	}
	\vspace{-1ex}
	\label{tbl:retrieval}
\end{table*}		
